On Text-based Personality Computing: Challenges and Future Directions

Text-based personality computing (TPC) has gained many research interests in NLP. In this paper, we describe 15 challenges that we consider deserving the attention of the research community. These challenges are organized by the following topics: personality taxonomies, measurement quality, datasets, performance evaluation, modelling choices, as well as ethics and fairness. When addressing each challenge, not only do we combine perspectives from both NLP and social sciences, but also offer concrete suggestions. We hope to inspire more valid and reliable TPC research.

==> writing/2Literature.tex <==
\section{Literature Search}
\label{sec_literature}
To search for relevant TPC studies in the ACL Anthology, we use the following search terms: “personality”, “personality prediction”, “personality computing” and “personality recognition”. The search date is August 29, 2022. We also sort the results by “relevance” and “year of publication”, separately, as these two options return different search results. For all the returned papers, we check their titles, abstracts and (when necessary) main texts, and retain those that fall under one of the following categories:

\paragraph{Dataset Type-A}
Papers focusing on introducing new datasets for TPC. Some also benchmark TPC models against new datasets. There are 7.

\paragraph{Dataset Type-B}
Papers that introduce datasets for non-TPC goals (e.g., multimodal PC, natural language generation, modelling laughter in conversations) but happen to include personality and text data that can be used for TPC. There are 5.

\paragraph{TPC as End}
Empirical papers where TPC is the main goal. There are 31.

\paragraph{TPC as Means}
Empirical papers where TPC is not the ultimate goal but used for further purposes like emotion detection, natural language generation and sociolinguistic analysis. There are 17.

We exclude papers that mean PC as the computing of personality disorders or personal profiles. In total, we find and review 60 TPC papers. See Appendix~\ref{sec:appendixA} for an overview of these papers sorted by their associated categories. Also, see Appendix~\ref{sec:appendixB} for 18 shareable TPC datasets that we find via these 60 papers. 
